Learning to Move with Affordance Maps

The ability to autonomously explore and navigate a physical space is a fundamental requirement for virtually any mobile autonomous agent, from household robotic vacuums to autonomous vehicles. Traditional SLAM-based approaches for exploration and navigation largely focus on leveraging scene geometry, but fail to model dynamic objects (such as other agents) or semantic constraints (such as wet floors or doorways). Learning-based RL agents are an attractive alternative because they can incorporate both semantic and geometric information, but are notoriously sample inefficient, difficult to generalize to novel settings, and are difficult to interpret. In this paper, we combine the best of both worlds with a modular approach that learns a spatial representation of a scene that is trained to be effective when coupled with traditional geometric planners. Specifically, we design an agent that learns to predict a spatial affordance map that elucidates what parts of a scene are navigable through active self-supervised experience gathering. In contrast to most simulation environments that assume a static world, we evaluate our approach in the VizDoom simulator, using large-scale randomly-generated maps containing a variety of dynamic actors and hazards. We show that learned affordance maps can be used to augment traditional approaches for both exploration and navigation, providing significant improvements in performance.

==> approach_new.tex <==
\section{Approach}
Our goal is to build an agent that can efficiently explore and navigate novel environments populated with other dynamic agents, while respecting the semantic constraints of the environment. 
We consider a mobile agent capable of executing basic movement macro-actions. This agent is equipped with a RGBD camera and some form of proprioceptive feedback indicating well-being (e.g bump sensor, wheel slip, game damage). As our focus is on semantic constraints, we assume that the agent is well localized, though our proposed approach can be used in conjunction with any off-the-shelf odometry system (such as \cite{mur2015orb}).

% Furthermore, the exact dimensions of the agent and affordances provided by entities in the environment are unknown.

\begin{figure}[ht]
  \centering
  \vspace{-5pt}
  \includegraphics[width=\linewidth]{./figs/arch_test.png}
  \vspace{-13pt}
  \caption{Overview of our proposed architecture for navigation. RGBD inputs $x_t$ are used to predict affordance maps $\hat{y_t}$ and transformed into egocentric navigability maps $M_t$ that incorporate both geometric and semantic information. The map shown in the figure labels the hallway with a monster as non-navigable. A running estimate of the current position at each time step is maintained and used to update a global, allocentric map of navigability $G_t$ that enables safe and efficient planning.}
  \vspace{-2pt}
  \label{fig:evaluation}
\end{figure}

% \deva{Make sure the definition of $y_$ as the {\em affordance} map and $M_t$ as the {\em navigability} map is consistent throughout paper (e.g., not true in Fig 2 or "navigability segmentation" in Sec 3.1).}
We propose a modular approach to tackling this problem. In particular, we adopt a classical pipeline of map building and path planning. Figure~\ref{fig:evaluation} shows the overview of our pipeline, where we use sensor observations to estimate traversability around the agent. This traversability is integrated over time to produce global maps, and navigation problems are solved via path-planning on these global maps. For an environment without any semantic constraints or dynamic other agents, this notion of traversability is entirely determined by geometry. This can be obtained directly via use of depth sensors.
However, when the environment has semantic constraints or dynamic objects, there is a mismatch between what parts of the environment are actually traversable versus what parts are traversable as per geometry. This motivates our approach, where we employ learning to improve traversability estimation in such situations. Our key contribution is the design of a self-supervision scheme to efficiently learn this traversability prediction function. We describe this Navigability Module next.

% Figure \ref{fig:evaluation} shows an overview of our approach to navigation, which builds a navigability map of the environment using both geometric and semantic information, as opposed to traditional methods that rely on geometry alone. One key component of our approach, shown in Figure~\ref{fig:sampling}, is a method for predicting which parts of a scene are navigable by actively leveraging the feedback sensor to generate partially-labeled training examples. We then use the labeled samples to train a model which predicts a per-pixel affordance map from the agent's viewpoint. At evaluation time, the outputs from the learned module are combined with geometric information from the depth sensor to build egocentric and allocentric representations that capture both semantic and geometric constraints. The fused representations can then be used for exploration and navigation by employing traditional path planning techniques to enable safe navigation even in dynamic and hazardous environments.

\subsection{Navigability Module} \label{navigability}
While we want to leverage learning to predict navigability, we also want to leverage geometry information available from on-board sensors as much as possible. Thus, instead of directly learning to predict top-down navigability maps from first person image observations, we instead make navigability predictions in the 2D image space. These navigability predictions are back-project into space using the measured geometry information to obtain top-view navigability predictions (much like \cite{henriques2018mapnet}). Given we assume that the agent can approximately measure geometry using onboard RGB-D sensors, this choice makes learning more sample efficient.

Thus, our learning task reduces to that of a 2D semantic segmentation task, where we want to label images into navigable regions, which when back-projected lead to navigability maps that respect semantic constraints of the environment, and motion of other dynamic agents. The next natural question is, how do we get training data for learning this navigability function? For typical semantic segmentation tasks, it is common in computer vision to gather large-scale labeled datasets~\citep{lin2014microsoft, cordts2016cityscapes}. Not only is this hard to scale, in our setup this is also challenging because navigability also depends on the behavior of other dynamic agents (which in-turn depends on the behavior of the agent). To tackle this issue, we propose a self-supervised scheme for automatically gathering these labels from interaction. This makes the labeling process scalable, as well as, well-grounded in context of the task and the environment.

% Given a scene representation $x$ captured by a RGBD camera, we want to train a module $\pi$ that labels each pixel with a binary affordance value, describing whether the corresponding position is a valid space for the agent to occupy and forming a segmentation map of ``navigability" $y$.  We can encode this understanding of the environment by training an image segmentation model in a supervised fashion. However, training such a model requires a set of labeled training images $D = [(x_1, y_1), ... (x_n, y_n)]$ where each pixel is annotated for navigability. Traditionally, obtaining such a set of labels has required dense annotation by an oracle \citep{cordts2016cityscapes}, at a cost that scales linearly with the amount of data labeled. These properties have generally limited applications to domains captured by large segmentation datasets \citep{lin2014microsoft, zhou2017scene} that have been painstakingly curated with hundreds of hours of human annotation time. 

\begin{figure}[ht]
  \vspace{-2mm}
  \centering
  \includegraphics[width=\linewidth]{./figs/arch_sample.png}
  \vspace{-2mm}
  \caption{Overview of self-supervised labeling for navigability training pairs $(\tilde{x}, \tilde{y})$. The agent performs a series of walks along random or planned trajectories within the environment. Affordance information collected from each walk is back-projected onto pixel-level labels in the agent's POV from previous time steps. Sampling over a variety of maps allows for the collection of a visually and semantically diverse set of examples $\tilde{D}$ that can be used to train a navigability module $\pi$. This figure illustrates the generation of a negative example, with the agent contacting a dynamic hazard.}
  \label{fig:sampling}
  \vspace{-2mm}
\end{figure}

\textbf{Self-Supervised Data Labeling.}
Our self-supervised data labeling algorithm uses RGBD observations $x$, readings from a feedback sensor $s$, and a history of actions $a_t$ executed over time. This data is gathered in the training environment, where we let the agent continuously interact with the environment. 
In each episode, the agent is randomly initialized at a random location, orientation in a random training environment. The agent selects a random nearby point and attempts to navigate towards it. Labeled training data is generated based on whether the agent is able to get this nearby point or not: every location that the agent successfully traverses during its attempt is marked as navigable, while undesirable locations (bumping into obstacles, loss of traction, loss in health, getting stuck) are marked as non-navigable. These location labels in top-view are projected into the image frame using the estimated camera intrinsics, to obtain segmentation labels. Figure~\ref{fig:samples} shows a visualization of this process. Pixels for which there are no positive or negative labels are marked as unknown. 

Though conceptually simple, backprojection of affordance labels produces a dense set of {\em pixelwise} labels at all time steps. This is in contrast to RL-based methods that return only a single sparse scalar reward, which often leads to sample inefficient learning requiring millions of sampling episodes~\citep{zhu2017target}. Furthermore, the generated labels are human interpretable, and provide an explanation for the actions taken by the agent.

\label{approach}
\begin{figure}[ht]
\centering
  \includegraphics[width=\linewidth]{./figs/sample_egs.png}
  %\vspace{-5pt}
  \caption{Examples of samples labeled through back-projection (navigable area labeled in green, non-navigable in yellow, and unknown in purple). The first three examples show negative examples, labeled by damage from monster, impediment of movement by barrel, and damage taken from environmental hazard respectively. The fourth illustrates successful traversal between monsters and the fifth shows an example collected along a minimum cost path as part of an active learning loop.}
%\vspace{-10pt}
\label{fig:samples}
\end{figure}

\textbf{Navigability Training.}
The collected samples (images with navigability labels) are used to train a semantic segmentation network (UNet \citep{ronneberger2015u}). We use a binary cross-entropy loss and only penalize the output where we observed positive of negative labels. \sg{William fix: We also weight each pixel's contribution inversely by the Euclidean distance from its associated label center.} Training on samples gathered from diverse training environments allows the navigability module to generalize well to previously unseen environments.


\textbf{Active trajectory sampling for faster learning.}
To improve sample efficiency further, we employ active learning to gather more effective paths for learning. 
Semantically interesting artifacts (such as as hazards) and other dynamic agents are rare, thus active seeking them out speeds up learning. We iterate between phases of model training, and active data gathering. We use the current navigability module and obtain estimates of the uncertainty in its prediction, by measuring the entropy of the module's output. Instead of back-projecting the labels, we back-project the \textit{inverse of this uncertainty} and use these as the cost-maps for path planning. Following a minimal-cost path in this space amounts to following the most uncertain path, leading to collection of more informative samples. We append this additional data to the dataset, and re-train to generate the next version of the model. Figure~\ref{fig:samples}(right) shows training samples sought out by our proposed active learning scheme.

\subsection{Map Construction}
Given navigability predictions on the 2D image, we back-project them into 3D space (using the onboard depth sensor) to obtain egocentric semantic navigability predictions, $M^s_t$, in the top-down view (that is used for path planning). We also use egocentric geometric navigability maps, $M^g_t$ (as obtained directly by back-projecting the depth image). We fuse $M^s_t$ and $M^g_t$ to produce a single local ego-centric map $M_t$ that captures both geometric and semantic constraints. We stitch these ego-centric maps $M_t$ together over time, to obtain global allocentric navigability maps $G_t$ at each time step. 

% \textbf{Map Fusion.}
% Given a pixel-wise affordance map $\hat{y}_t$ obtained from the navigability module and a local, egocentric geometric map $M^G_t$, the two inputs can be combined using a fusion module $F(\hat{y}_t, M^G_t)$ to form a single local navigation cost map $M_t$ that incorporates both semantic and geometric information. To do so, the segmentation map $\hat{y}_t$ is first projected into the 2D plane using estimated camera intrinsics, forming an egocentric affordance map $M^S_t$. Cells marked as obstacles by $M^G_t$ are also marked as impassable within $M_t$, with remaining cells in free space assigned cost values proportional to the confidence of non-navigability provided by $\hat{y}_t$. Finally, $M_t$ is used to update a global, allocentric map $G_t$ of navigability at the end of each time step.

\subsection{Planning}
Given the global navigability map, path planning is done via classical path planning algorithms such as $A*$. All geometric and semantic information about the environment is represented within the map, thus the overall behavior respect semantic constraints of the environment. Since both $M_t$ and $G_t$ are updated at every time step, dynamic hazards are treated as any other obstacle and can be avoided successfully by replanning paths at sufficiently high frequency. Our work is agnostic to the choice of the path planners, and our semantic maps can as well be used with more sophisticated path planners, though for simplicity we show results with $A*$.
%\deva{I think we should explicitly state that we use a frontier planner for exploration and A* planner for navigation.}

